Generalised hyperbolicity in conical space-times

Solutions of the wave equation in a space-time containing a thin cosmic string are examined in the context of non-linear generalised functions. Existence and uniqueness of solutions to the wave equation in the Colombeau algebra G is established for a conical space-time and this solution is shown to be associated to a distributional solution. A concept of generalised hyperbolicity, based on test fields, can be defined for such singular space-times and it is shown that a conical space-time is G-hyperbolic.

==> crossref.tex <==

%% Numbering and cross referencing for Plain TeX and AMS-TeX
%% J.P.Wilson

\catcode`\@=11

\newwrite\auxout
\newif\ifauxopen
\newif\iffileexists
\def\gobble#1{}
\def\typeout{\immediate\write16}

\chardef\letter=11
\def\setletters{%
  \catcode`_=\letter \catcode`+=\letter
  \catcode`-=\letter \catcode`@=\letter
  \catcode`0=\letter \catcode`1=\letter
  \catcode`2=\letter \catcode`3=\letter
  \catcode`4=\letter \catcode`5=\letter
  \catcode`6=\letter \catcode`7=\letter
  \catcode`8=\letter \catcode`9=\letter
  \catcode`(=\letter \catcode`)=\letter
  \catcode`:=\letter \catcode`'=\letter
  \catcode`&=\letter \catcode`;=\letter
  \catcode`.=\letter}%

% File handling controls

\outer\def\crossreferencing{%
 \begingroup
 \immediate\openin0=\jobname.aux\space
 \ifeof0 \global\fileexistsfalse
  \typeout{Creating file \jobname.aux}
  \else\global\fileexiststrue\fi
 \immediate\closein0\endgroup
 \iffileexists\begingroup\setletters
   \input \jobname.aux \endgroup \fi
 \immediate\openout\auxout=\jobname.aux
   \typeout{Writing to \jobname.aux}
   \auxopentrue}%

\def\closeallfiles{\ifauxopen\immediate\closeout\auxout\fi}
\outer\def\bye{\par\vfill\supereject\closeallfiles\end}

% Write out the last generated number to the .aux file

\def\xlabel#1{\ifauxopen \begingroup\setletters 
 \expandafter\xdef\csname XR#1\endcsname{\xrflabel}%
 \immediate\write\auxout{\string\gdef
   \expandafter\string\csname XR#1\endcsname{\xrflabel}}% 
\endgroup\ignorespaces\fi}%
\def\setlabel#1{\global\let\xrflabel=#1}
\def\stepsetlabel#1#2{\stepup{#1}\setlabel{#2}#2}
\setlabel\null

% Write the current page number out to the .aux file

\def\xpagelabel#1{\ifauxopen \begingroup\setletters
 \expandafter\xdef\csname XR#1\endcsname{\folio}%
 \write\auxout{\string\gdef
   \expandafter\string\csname XR#1 \endcsname{\folio}}% 
\endgroup\ignorespaces\fi}%

% Read the cross reference

\def\xref#1{\begingroup\setletters
 \expandafter\ifx \csname XR#1\endcsname \relax
   \typeout{Warning: Label `#1' undefined}%
    \expandafter\gdef \csname XR#1\endcsname{00}%
  \else \csname XR#1\endcsname
\fi\endgroup}

\def\reset#1{\global#1=0}
\def\stepup#1{\global\advance#1by1}
\def\stepdown#1{\global\advance#1by-1}

% Define counters suitable for numbering a journal paper

\newcount\eqcount      % equations
\newcount\seccount     % sections
\newcount\proccount    % proclaims
\newcount\defcount     % definitions

\def\eqprint{\number\eqcount}
\def\secprint{\number\seccount}
\def\procprint{\number\proccount}
\def\defprint{\number\defcount}

% The \appendix control sequence should appear before the first
% appendix. The counters are reset with `A' appended to them

\outer\def\appendix{%
  \reset\eqcount   \def\eqprint{A.\number\eqcount}%
  \reset\seccount  \def\secprint{A.\number\secprint}%
  \reset\proccount \def\procprint{A.\number\procprint}%
  \reset\defcount  \def\defprint{A.\number\defprint}%
}

% Generators for the numbers. The control sequences advance the counters,
% copy their values to the cross reference register and print them out.

% \eqnum should be used in conjunction with \eqno, \leqno, \eqalignno or
% \leqalignno and not with an AMS-TeX alignment such as \alignat. The
% other generators should work well with both plain TeX or AMS-TeX macros

\def\eqnum{\stepup\eqcount\setlabel\eqprint(\eqprint)}
\def\secnum{\stepup\seccount\setlabel\secprint\secprint}
\def\procnum{\stepup\proccount\setlabel\procprint\procprint}
\def\defnum{\stepup\defcount\setlabel\defprint\defprint}
\def\eqref#1{{\rm(}\xref{#1}{\rm)}}

% Support for AMS-TeX alignments such as \alignat and \xalignat

% There appears to be  a problem with using automatically numbered
% equations in  AMS-TeX's alignment structures, because macros such as
% \alignat actually  processes the equations  twice; the first pass
% measures the equations where as the second pass actually prints them;
% therefore the equation counter could advance during the  measurement pass
% and two duplicate cross reference entries written. 

% The solution is suppress the advancing of \equationno and the writing of 
% cross references during the measurement pass.

% The \tagnum control sequence should be used in ALL AMS-TeX alignment
% structures immediately after a \tag. It may of course be followed by an
% \xlabel control sequence.

\let\x@label=\xlabel
\def\tagnum{{\ifmeasuring@\global\let\xlabel=\gobble
    \else\global\let\xlabel=\x@label\stepup\eqcount\setlabel\eqprint
  \fi\eqprint}}



\catcode`\@=12
\endinput












